A new short proof of regularity for local weak solutions for a certain class of singular parabolic equations

We shall establish the interior H\"older continuity for locally bounded weak solutions to a class of parabolic singular equations whose prototypes are \begin{equation} u_t= \nabla \cdot \bigg( |\nabla u|^{p-2} \nabla u \bigg), \quad \text{ for } \quad 1<p<2, \end{equation} and \begin{equation} u_{t}- \nabla \cdot ( u^{m-1} | \nabla u |^{p-2} \nabla u ) =0 , \quad \text{for} \quad m+p>3-\frac{p}{N}, \end{equation} via a new and simplified proof using recent techniques on expansion of positivity and $L^{1}$-Harnack estimates.

==> dibe_0307 <==
%%n if using the Springer package svmno.cls the 
%% theorem envronment is already defined
%% if not remove the comment below

%%%%%%%%%% LEMMA, THM, PROP, SECTION %%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
%\newtheorem{proof}{Proof}

\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
\numberwithin{equation}{section}
\numberwithin{theorem}{section}
\numberwithin{proposition}{section}
\numberwithin{lemma}{section}
\numberwithin{remark}{section}
\setcounter{secnumdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% FORMATTING MACROS %%%%%%

\newcommand{\cl}{\centerline}
\newcommand{\sms}{\smallskip}
\newcommand{\ms}{\medskip}
\newcommand{\bs}{\bigskip}
\newcommand{\noi}{\noindent}
\newcommand{\itl}[1]{\textit{#1}}
\newcommand{\blf}[1]{\textbf{#1}}
\newcommand{\dsty}{\displaystyle}
\newcommand{\txty}{\textstyle}
\newcommand{\ssty}{\scriptstyle}
\newcommand{\tty}{\texttt}

%%%%%%%%%% SPECIAL SYMBOLS %%%%%%%%%%%%

\newcommand\Par{\mathhexbox278\,}

%%%% GREEK LETTERS  %%%%%%%%

\newcommand{\al}{\alpha}
\newcommand{\Al}{\Alpha}
\newcommand{\be}{\beta}
\newcommand{\Be}{\Beta}
\newcommand{\Gm}{\Gamma}
\newcommand{\gm}{\gamma}
\newcommand{\dl}{\delta}
\newcommand{\Dl}{\Delta}
\newcommand{\lm}{\lambda}
\newcommand{\Lm}{\Lambda}
\newcommand{\kp}{\kappa}
\newcommand{\varep}{\varepsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\vp}{\varphi}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\uom}{\mbox{\boldmath$\omega$}}
\newcommand{\btau}{\mbox{\boldmath$\tau$}}
\newcommand{\bnu}{\mbox{\boldmath$\nu$}}
\newcommand{\up}{\upsilon}
\newcommand{\z}{\zeta}


%%% SPECIAL MATH SYMBOLS %%%%%%%%%%%%

\newcommand{\df}[1]{\buildrel\mbox{\small def}\over{#1}}
\newcommand{\op}[1]{\buildrel\mbox{\tiny o}\over{#1}}
\newcommand{\db}{\prime\prime}
\newcommand{\bsl}{\backslash}
\newcommand{\lb}{\lbrack\!\lbrack}
\newcommand{\rb}{\rbrack\!\rbrack}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand{\ev}{\equiv}
\newcommand{\nev}{\not\equiv}
\newcommand{\nn}{\mathbb{N}}
\newcommand{\qq}{\mathbb{Q}}
\newcommand{\zz}{\mathbb{Z}}
\newcommand{\rr}{\mathbb{R}}
\newcommand{\rn}{\rr^N}
\newcommand{\cc}{\mathbb{C}}
\newcommand{\id}{\mathbb{I}}
\newcommand{\bo}{\mathbb{O}}

\newcommand{\amsb}[1]{\mathbb{#1}}
\newcommand{\mcl}[1]{\mathcal{#1}}
\newcommand{\bl}[1]{\mathbf{#1}}
%\newcommand{\blm}[1]{\boldsymbol{#1}}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}

\newcommand{\lra}{\longrightarrow}
\newcommand{\LLR}{\Longleftrightarrow}
\newcommand{\LRA}{\Longrightarrow}
\newcommand{\LLA}{\Longleftarrow}

%%%% BLACK BOX AND OPEN BOX %%%%%%%%%%%%%%%%

\newcommand{\bbox}{\vrule height.6em width.6em 
depth0em} %%%%% Black Box
\newcommand{\os}{\vbox{\hrule \hbox{\vrule 
height.6em depth0pt 
\hskip.6em \vrule height.6em depth0em}
\hrule}} %%%%%% Open Square

%%%%%%%%%%%%%% OPERATORS %%%%%%%%%%%%%%%%%%%

%\newcommand{\ker}{\operatorname{ker}}
\newcommand{\dvg}{\operatorname{div}}
\newcommand{\curl}{\operatorname{curl}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\essup}{\operatornamewithlimits{ess\,sup}}
\newcommand{\essinf}{\operatornamewithlimits{ess\,inf}}
\newcommand{\essosc}{\operatornamewithlimits{ess\,osc}}
\newcommand{\osc}{\operatornamewithlimits{osc}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\loc}{\operatorname{loc}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\meas}{\operatorname{meas}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\dtm}{\operatorname{det}}
%

%%%%%%%% OVER AND UNDER LIMITS %%%%%%%%%%%

\newcommand{\overlim}{\mathop{\overline{\lim}}\limits}
\newcommand{\underlim}{\mathop{\underline{\lim}}\limits}
\newcommand{\ttop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
%\newcommand{\trtop}[3]{\genfrac{}{}{0pt}{}{#1}{#2}{#3}}
%\newcommand{\trtop}[3]{\genfrac{}{}{}{0pt}{}{#1}{#2}{#3}}
\newcommand{\bcu}{\mathop{\txty{\bigcup}}\limits}
\newcommand{\bca}{\mathop{\txty{\bigcap}}\limits}
\newcommand{\bsu}{\mathop{\txty{\sum}}\limits}
\newcommand{\pro}{\mathop{\txty{\prod}}\limits}


%%%%%%%%%%%  DERIVATIVES %%%%%%%%%%%%%%%%

\newcommand{\pl}{\partial}
\newcommand{\ptt}{\frac{\pl}{\pl t}}
\newcommand{\ppx}{\frac\pl{\pl x}}
\newcommand{\dds}{\frac d{ds}}
\newcommand{\ddt}{\frac d{dt}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  INTEGRALS  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\intl}{\int\limits}
\newcommand{\iintl}{\iint\limits}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  INTEGRAL AVERAGES  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Xint#1{\mathchoice
    {\XXint\displaystyle\textstyle{#1}}%
    {\XXint\textstyle\scriptstyle{#1}}%
    {\XXint\scriptstyle\scriptscriptstyle{#1}}%
    {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
    \!\int}
\def\XXint#1#2#3{\setbox0=\hbox{$#1{#2#3}{\int}$}
    \vcenter{\hbox{$#2#3$}}\kern-0.5\wd0}
\def\bint{\Xint-}
\def\dashint{\Xint{\raise4pt\hbox to7pt{\hrulefill}}}

% integral averages

\newcommand{\ovl}[3]{\int_{#1}^{#2}\kern-#3pt\raise4pt\hbox to7pt{\hrulefill}\ }

\newcommand{\ovll}[3]{\intl_{#1}^{#2}\kern-#3pt\raise4pt\hbox to7pt{\hrulefill}\ }

\newcommand{\tvl}[2]{\iint_{#1}\kern-#2pt\raise4pt\hbox to15pt{\hrulefill}\ }

%%%%%%%%%%% ANALYSIS MACROS %%%%%%%%%%%%%%%%%%%

%%%% Domain \Om %%

\newcommand{\omt}{\Om_T}
\newcommand{\plo}{\partial\Omega}
%\newcommand{\ovo}{\overline{\Om} }
\newcommand{\ovo}{\bar{\Om} }

%% C-infinity Local spaces and symbols
%
\newcommand{\ci}[1]{C^\infty\!\left({#1}\right)}
\newcommand{\cio}[1]{C_o^\infty\!\left({#1}\right)}
\newcommand{\lloc}[1]{L_{\loc}\!\left({#1}\right)}
\newcommand{\xy}{|x-y|}

%% Integrals

\newcommand{\intom}{\intl_{\Om}}
\newcommand{\intbo}{\intl_{\plo}}
\newcommand{\inom}{\int_{\Om}}
\newcommand{\inbo}{\int_{\plo}}
\newcommand{\intrn}{\intl_{\rn}}

%%%%%%%%%%%% ENDING THE DOCUMENT %%%%%%%%%%%%%%%%

\newcommand{\bye}{\end{document}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\hsize=5in
%\vsize=7.5in

%
%% Tag
%
%\def\uptag#1#2$${\iftagsleft@\leqno\else\eqno\fi
%  \hbox{\def\pagebreak{\global\postdisplaypenalty-\@M}%
%  \def\nopagebreak{\global\postdisplaypenalty\@M}\rm(#1\unskip)${}^{#2}$}%
%  $$\postdisplaypenalty\z@\ignorespaces}
%

%\def\btag#1#2$${\iftagsleft@\leqno\else\eqno\fi
%  \hbox{\def\pagebreak{\global\postdisplaypenalty-\@M}%
%  \def\nopagebreak{\global\postdisplaypenalty\@M}\rm(#1\unskip)${}_{#2}$}%
%  $$\postdisplaypenalty\z@\ignorespaces}
%
%\def\ubtag#1#2#3$${\iftagsleft@\leqno\else\eqno\fi
%  \hbox{\def\pagebreak{\global\postdisplaypenalty-\@M}%
%  \def\nopagebreak{\global\postdisplaypenalty\@M}
%  \rm(#1\unskip)${}_{#2}^{#3}$}%
%  $$\postdisplaypenalty\z@\ignorespaces}
%
%\def\ptag#1$${\iftagsleft@\leqno\else\eqno\fi
%  \hbox{\def\pagebreak{\global\postdisplaypenalty-\@M}%
%  \def\nopagebreak{\global\postdisplaypenalty\@M}
%  \rm(#1\unskip)${}^{\prime}$}%
%  $$\postdisplaypenalty\z@\ignorespaces}
%
%% tag wih no brackets
%
%\def\etag#1$${\iftagsleft@\leqno\else\eqno\fi
%  \hbox{\def\pagebreak{\global\postdisplaypenalty-\@M}%
%  \def\nopagebreak{\global\postdisplaypenalty\@M}\rm#1\unskip}%
%  $$\postdisplaypenalty\z@\ignorespaces}
%


%%%%%% DEFINIZIONE DI DATA GIORNO, MESE, ANNO %%%%%%%%%%
%
%\newcommand{\data}{\number\day\space \ifcase\month\or
%Gennaio\or Febbraio\or Marzo\or Aprile\or Maggio\or 
%Giugno\or
%Luglio\or Agosto\or Settembre\or Ottobre\or Novembre\or
%Dicembre\fi,\space\number\year}
%


